URLLC with Massive MIMO: Analysis and Design at Finite Blocklength

The fast adoption of Massive MIMO for high-throughput communications was enabled by many research contributions mostly relying on infinite-blocklength information-theoretic bounds. This makes it hard to assess the suitability of Massive MIMO for ultra-reliable low-latency communications (URLLC) operating with short blocklength codes. This paper provides a rigorous framework for the characterization and numerical evaluation (using the saddlepoint approximation) of the error probability achievable in the uplink and downlink of Massive MIMO at finite blocklength. The framework encompasses imperfect channel state information, pilot contamination, spatially correlated channels, and arbitrary linear spatial processing. In line with previous results based on infinite-blocklength bounds, we prove that, with minimum mean-square error (MMSE) processing and spatially correlated channels, the error probability at finite blocklength goes to zero as the number $M$ of antennas grows to infinity, even under pilot contamination. On the other hand, numerical results for a practical URLLC network setup involving a base station with $M=100$ antennas, show that a target error probability of $10^{-5}$ can be achieved with MMSE processing, uniformly over each cell, only if orthogonal pilot sequences are assigned to all the users in the network. Maximum ratio processing does not suffice.

==> defs.tex <==
\usepackage{bm}
\usepackage{upgreek}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage{xspace}

\safemath{\mi}{I}
\safemath{\difent}{\mathrm{h}}		%differential entropy
\safemath{\NonnegReal}{\mathbb{R}^{+}}


\safemath{\indist}{\cdfP} %input distribution
\safemath{\outdist}{\cdfQ} %output distribution
\safemath{\inpdf}{\pdfp} %input pdf
\safemath{\outpdf}{\pdfq} %output pdf
\safemath{\testdist}{\cdfP} %the distribution of test P_{Z|W}

%\safemath{\tr}[#1]{\mathrm{tr}\left\lbrace #1  \right\rbrace}

\safemath{\powallocvec}{\vecv}
\safemath{\powalloc}{v}
\safemath{\encoder}{f} % the encoder of the code
\safemath{\decoder}{g} % the decoder of the code
\safemath{\msg}{J} % the message
\safemath{\csir}{\mathrm{r}}
\safemath{\csit}{\mathrm{t}}
\safemath{\csi}{\mathrm{csi}}
\safemath{\csirt}{\mathrm{rt}}
\safemath{\Rcsirt}{R_{\csirt}} %rate with CSIT
\safemath{\Rcsir}{R_{\csir}}
\safemath{\Rcsit}{R_{\csit}}
\safemath{\cohblock}{T}
\safemath{\blocklength}{n}
\safemath{\selbranches}{L}


\safemath{\Rnocsit}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rnocsi}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rgeneral}{R_{\mathrm{no,rt}}} %rate with general CSI condition
\safemath{\equalR}{R_{\mathrm{e}}}

\newcommand*\pFqskip{8mu}
\catcode`,\active
\newcommand*\pFq{\begingroup
        \catcode`\,\active
        \def ,{\mskip\pFqskip\relax}%
        \dopFq
}
\catcode`\,12
\def\dopFq#1#2#3#4#5{%
        {}_{#1}F_{#2}\biggl[\genfrac..{0pt}{}{#3}{#4};#5\biggr]%
        \endgroup
}

%------------------------------------
%		JOHAN
%------------------------------------
\safemath{\Rmax}{R^*(n,\epsilon)} %rate without CSIT
\safemath{\codewords}{K}
\safemath{\Rub}{\bar{R}(n,\epsilon)}
\safemath{\Rlb}{\underline{R}(n,\epsilon)}
\safemath{\rk}{\kappa}
\safemath{\rlos}{\bar{\matH}}
\safemath{\rnlos}{\tilde{\randmatH}}

\safemath{\randtemp}{K}

\safemath{\Vnocsit}{V_{\error}^{\mathrm{no}}}
\safemath{\Vcsit}{V_{\error}^{\mathrm{rt}}}

\safemath{\cadist}{F_C} %capacity distribution
\safemath{\cdistno}{F_{0}}
\safemath{\cdistcsit}{F_{1}}


\safemath{\deF}{d_0} %the derivative of F_C(\xi) %\left.\frac{d\cadist(\argpn)}{d\argpn}\right|_{\argpn=C_\error}

\safemath{\bl}{n} %block length
\safemath{\blt}{\tilde{\bl}}
\safemath{\error}{\epsilon} %prob of error
\safemath{\NumCode}{M}
\safemath{\RXant}{r}
%\safemath{\rxant}{r}
%\safemath{\txant}{t}
\safemath{\txantop}{t^{\ast}}
\safemath{\minant}{m}
\safemath{\minantop}{\minant^\ast}
\safemath{\snr}{\rho}
\safemath{\const}{k}
\safemath{\inset}{\setF} %the input power set
\safemath{\spanm}{\mathrm{span}}
\safemath{\ubb}{b_{0}}%upper bound of b_1,...,b_{r} of the matrix I+ H^H U H.

%%%%%%%%%%%MIMO%%%%%%%%%%%%%%%%%%%%
\safemath{\covmat}{\matU}
\safemath{\covmatY}{\matV}
\safemath{\randcmY}{\randmatV}

\safemath{\insetMIMO}{\setF_{\txant,\bl}}
\safemath{\insetcov}{\setU_{\txant}}
%\safemath{\condcov}{\matQ\succeq\mathbf{0},\tr(\matQ)\leq\snr}
\safemath{\condcov}{\matQ\in\insetcov}

\safemath{\BoundFU}{k_{\delta}}

\safemath{\argpn}{\xi} % the argument in the probability p(R)

\safemath{\angletest}{Z} %the angle test used in achievability part

\safemath{\Cnocsit}{C_{\epsilon}^{(0)}}
\safemath{\Ccsit}{C_{\epsilon}^{(1)}}

\safemath{\errorach}{P_\mathrm{e}} %the error in intuition part



\newcommand{\given}{\,\vert\,}				% conditioning
\newcommand{\ggiven}{\,\Vert\,}
\safemath{\define}{\triangleq}			% definition
%\safemath{\fnorm}{\mathrm{F}}

\safemath{\altbl}{\tilde{\bl}}
\safemath{\constL}{k_{\mathrm{L}}}
\safemath{\constU}{k_{\mathrm{U}}}
\safemath{\funcL}{\tilde{q}}
\safemath{\funcU}{q}
\safemath{\ConstThm}{k_0}
%%%%%%%%%%%%%%%%used in the intuition part %%%%%%%%%%%%%
\safemath{\randrevec}{\randvecy}
\safemath{\revec}{\vecy}
\safemath{\trcwd}{\vecx}
\safemath{\randtrcwd}{\randvecx}
\safemath{\randnoisevec}{\randvecw}
\safemath{\transmitcwd}{\vecx_1} %the transmitted codeword in achievability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%used in the appendix of proving gamma=C_error + O(1/\bl) %%%%%%%%%%%%%
\safemath{\pickcwdnoch}{\vecx_0} %the chosen codeword x=[P,P,...,P]
\safemath{\pickcwd}{\vecx_0} %the chosen codeword x=[P,P,...,P]

\safemath{\inseqrand}{\randvecx}
\safemath{\inseq}{\vecx}

\safemath{\outseq}{\matY}
\safemath{\outseqrand}{\randmatY}

%used in the appendix of the proof of achievability
\safemath{\altT}{\widetilde{T}}
\safemath{\altU}{\widetilde{U}}
\safemath{\altmean}{\tilde{\mu}}
\safemath{\altvar}{\tilde{\sigma}}
\safemath{\altf}{\funcL}
\safemath{\altg}{\tilde{g}}
\safemath{\altgamma}{\tilde{\gamma}}
\safemath{\altdelta}{\tilde{\delta}}
\safemath{\altk}{\tilde{k}}
\safemath{\altconst}{\altk}
\safemath{\altbmLambda}{\widetilde{\bm{\Lambda}}}
\safemath{\constant}{\tilde{k}}
\safemath{\ntot}{n\sub{tot}}

